Related by Similarity II: Poncelet 3-Periodics in the Homothetic Pair and the Brocard Porism

Previously we showed the family of 3-periodics in the elliptic billiard (confocal pair) is the image under a variable similarity transform of poristic triangles (those with non-concentric, fixed incircle and circumcircle). Both families conserve the ratio of inradius to circumradius and therefore also the sum of cosines. This is consisten with the fact that a similarity preserves angles. Here we study two new Poncelet 3-periodic families also tied to each other via a variable similarity: (i) a first one interscribed in a pair of concentric, homothetic ellipses, and (ii) a second non-concentric one known as the Brocard porism: fixed circumcircle and Brocard inellipse. The Brocard points of this family are stationary at the foci of the inellipse. A key common invariant is the Brocard angle, and therefore the sum of cotangents. This raises an interesting question: given a non-concentric Poncelet family (limited or not to the outer conic being a circle), can a similar doppelg\"anger always be found interscribed in a concentric, axis-aligned ellipse and/or conic pair?

==> _not_used/220_app_brocard_relations.tex <==
In \cite[Eqs. 5 and 6]{bradley2007-brocard} two important relations are mentioned, the first one due to Shail \cite{shail1996-brocard}:

\begin{align}
    {d}=&2R\sin{\omega}\sqrt{1-4\sin^2{\omega}} \label{eqn:broc-dist} \\
    {|\Omega_1{X_3}|}=&R\sqrt{1-4\sin^2{\omega}} \label{eqn:b1x3} \\
    {|{X_3}{X_6}|}=&R\sqrt{1-3\tan^2{\omega} \label{eqn:x3x6}}
\end{align}

Position $\Omega_1,\Omega_2$ on the $x$ axis (this determines $d$), and select an $R{\geq}2d$ (minimum $R$ is derived in \cite[Eqs. 15--17]{shail1996-brocard}). In \eqref{eqn:broc-dist} solve for $\sin^2\omega$, i.e., $4 x(1-x)=k$, where $k=(d/R)^2<1/4$. Namely:

\[\sin^2{\omega}= \frac{1}{8} \left(1\pm\sqrt{1-4 k}\right)\]

With \eqref{eqn:b1x3} \eqref{eqn:x3x6} position $X_3$ and $X_6$ on the Brocard axis. The circle centered on $X_3$ and of radius $R$ will be the fixed circumcircle. Position one vertex $V_1=X_3+(0,R)$.

Recall that third vertex of a set of triangles with fixed base (length $s_1$) and Brocard angle $\omega$ describes a Neuberg Circle whose maximum and minimum altitude-by-base ratio $h/s_1$ are \cite[Neuberg Circles, Eqs. 6 and 7]{mw}:

\begin{equation}
\frac{h}{s_1}=\frac{1}{2}\left(\cot{\omega}\pm\sqrt{\cot^2{\omega}-3}\right)
\end{equation}

Since all are determined, we can find the isosceles triangle inscribed in the circle of radius $R$, centered on $X_3$, with $V_1=X_3+(0,R)$ and $h/s_1$ as above. Namely, $V_2, V_3 =...$.



==> _not_used/240_app_first_brocard.tex <==
Shown in Figure~\ref{fig:brocard-basic} (right) os the First Brocard Triangle (FBT). Its vertices are known to be concyclic\footnote{The circumcenter and symmedian point also lie on it \cite[Brocard Circle]{mw}.} with the two Brocard points \cite[First Brocard Triangle]{mw} on the Brocard Circle \cite[Brocard Circle]{mw}. 

Referring to Figure~\ref{fig:first-brocard-locus}:

\begin{proposition}
Over 3-periodics in the homothetic pair, the locus of the vertices of the FBT is an axis-aligned, concentric ellipse, homothetic to the ones in the pair and interior to the caustic.
\end{proposition}

\begin{proof}
\textcolor{red}{ronaldo}
\end{proof}

\begin{proposition}
Over 3-periodics in the homothetic pair, the area of the the FBT is invariant and given by
\[ {\frac {3\sqrt{3} ab\left( {a}^{2}-{b}^{2} \right) ^{2}  }{16
 \left( {a}^{2}+{b}^{2} \right) ^{2}}}
\]
\textcolor{red}{ronaldo}
\end{proposition}

\begin{proof}
\textcolor{red}{ronaldo}
\end{proof}

Since the FBT is known to be inversely similar to the reference triangle \cite[Inversely Similar]{mw}:

\begin{corollary}
The similarity ratio of homothetic 3-periodics to the FBT is invariant and given by
\[ \frac{ 2(a^2+b^2)}{ a^2-b^2}\cdot\]
\textcolor{red}{ronaldo} 
\label{cor:sim-ratio}
\end{corollary}

\subsection{Vertices of the FBT over the homothetic family}

These are given by:

\begin{align*}
br_1=& \frac{a^2-b^2}{2(a^2+b^2)} R_x B\\
%=&[{\frac {a \left( \sin \left( u \right) \sqrt {3}+\cos \left( u
% \right)  \right)  \left( {a}^{2}-{b}^{2} \right) %}{4\,{a}^{2}+4\,{b}^
%{2}}},{\frac {b \left( \cos \left( u \right) \sqrt {3}-\sin \left( u\right)  \right)  \left( {a}^{2}-{b}^{2} \right) }{4\,{a}^{2}+4\,{b}^
%{2}}} ]\\
br_2=&\frac{a^2-b^2}{2(a^2+b^2)} R_xC\\
%&[-{\frac {a \left( \sin \left( u \right) \sqrt {3}-\cos \left( u
 %\right)  \right)  \left( {a}^{2}-{b}^{2} \right) }{4\,{a}^{2}+4\,{b}^
%{2}}},-{\frac {b \left( \cos \left( u \right) \sqrt {3}+\sin %\left( u
% \right)  \right)  \left( {a}^{2}-{b}^{2} \right) }{4\,{a}^{2}+4\,{b}^
%{2}}}]\\
br_3=&\frac{a^2-b^2}{2(a^2+b^2)} R_x A
%&[{\frac {-a \left(  {a}^{2}-{b}^{2} \right) \cos \left( u \right) }{2\,
%{a}^{2}+2\,{b}^{2}}},{\frac {b\sin \left( u \right)  \left( {a}^{2}-{b
%}^{2} \right) }{2\,{a}^{2}+2\,{b}^{2}}}]
%
\end{align*}

where $R_x(x,y)=(-x,y)$ is a reflection.

\subsection{Brocard Circle}

Recall the Brocard circle is the circumcircle of the FBT \cite[Brocard Circle]{mw}.

\begin{corollary} Over 3-periodics in the homothetic pair, the ratio of areas of the circumcircle of 3-periodics to that of the Brocard circle is invariant and given by
\[  \frac{4(a^2+b^2)^2}{(a^2-b^2)^2} \cdot\]
\end{corollary}

\begin{proof}
The result follows from Corollary~\ref{cor:sim-ratio}. Straightforward calculations yield that the circumradius of 3-periodics is given by: 
\[ R^2= -\frac{(a^2-b^2)^3 \cos(6 t)}{32a^2b^2}+\frac{(a^2+b^2)(a^4+14a^2b^2+b^4)}{32a^2b^2}.\]
\end{proof}

\begin{proposition}
Over the homothetic family, the Brocard circle is given by:

\[ E(x,y)= \,{\frac { 4\left( {a}^{2}+{b}^{2} \right) ^{2}{x}^{2}}{{a}^{2}
 \left( a^2-b^2 \right) ^{2}  }}+ \,{\frac {4 \left( 
{a}^{2}+{b}^{2} \right) ^{2}{y}^{2}}{{b}^{2} \left( a^2-b^2 \right) ^{2}}}-1
\]
\end{proposition}


